PerfCurator: Curating a large-scale dataset of performance bug-related commits from public repositories

Performance bugs challenge software development, degrading performance and wasting computational resources. Software developers invest substantial effort in addressing these issues. Curating these performance bugs can offer valuable insights to the software engineering research community, aiding in developing new mitigation strategies. However, there is no large-scale open-source performance bugs dataset available. To bridge this gap, we propose PerfCurator, a repository miner that collects performance bug-related commits at scale. PerfCurator employs PcBERT-KD, a 125M parameter BERT model trained to classify performance bug-related commits. Our evaluation shows PcBERT-KD achieves accuracy comparable to 7 billion parameter LLMs but with significantly lower computational overhead, enabling cost-effective deployment on CPU clusters. Utilizing PcBERT-KD as the core component, we deployed PerfCurator on a 50-node CPU cluster to mine GitHub repositories. This extensive mining operation resulted in the construction of a large-scale dataset comprising 114K performance bug-fix commits in Python, 217.9K in C++, and 76.6K in Java. Our results demonstrate that this large-scale dataset significantly enhances the effectiveness of data-driven performance bug detection systems.

==> 00_workload.tex <==
\balance
\newpage

\begin{table*}
\begin{tabular}{|l|l|l|l|}
\hline
\textbf{Content} & \textbf{Pages} & \textbf{Author} & \textbf{Complete?} \\ \hline
0. Abstract & 0.5 & Probir & 80\% \\ \hline
1. Introduction & 1.5 & Probir & 90\% \\ \hline
2. Background and Related work & 0.5 & Azad & No \\ \hline
2. RQ1 & 1 & Probir & 90\% \\ \hline
\textcolor{red}{3. RQ2} & 2 & \textcolor{red}{Azad} & \textcolor{red}{96\%} \\ \hline
4. RQ3 & 1 & Probir & 90\% \\ \hline
\textcolor{red}{5. RQ4} & 1.5 & \textcolor{red}{Azad} & \textcolor{red}{60\%} \\ \hline
6. RQ5 & 0.75 & Foyzul & 100\% \\ \hline
7. \textcolor{red}{Discussion} & 0.25 & \textcolor{red}{Probir} & \textcolor{red}{0\%} \\ \hline
\textcolor{red}{8. Threats to Validity} & 0.5 & \textcolor{red}{Azad} & \textcolor{red}{No} \\ \hline
9. \textcolor{red}{Conclusions} & 0.25 & \textcolor{red}{Azad} & \textcolor{red}{No} \\ \hline
\end{tabular}
\caption{Workload Assignment}
\end{table*}
\balance
\newpage

==> 3.1_RQ3_old.tex <==

\section{RQ3: Computational overhead}
\label{section:methodology}
\Manoj{IN PROGRESS}\Azad{will merge with rq1, repetitive parts} Figure X(Bench-marking Results of the Performance Commit classification) shows the different Model performance during Bench-marking. 

\subsubsection{Dataset setup:} 
To Evaluate the Language Models performance on Implicit features and explicit features, we have tailored a 500 hand labelled dataset by two experts. we have manually picked complex cases where it requires in-depth knowledge to decide whether performance commit or non-performance commit. our validation gold labels have 250 performance commits and 250 non-performance commit. we have used this gold label to Evaluate the Language Model performances on the validation dataset. We have used 2x4090 server for our experimentation.

\Azad{I'll remove repeatation}Our Regex based approach, We have taken 8M commit messages then we have filtered them using our 41 Regex functions to capture the Performance Commits, we were able achieve 65.6\% accuracy in this method. we wanted a concrete approach to understand the commit messages we have used Roberta model. Since our data is unlabelled, we have used Heuristic Supervision approach to capture the Performance and Non-performance Regexes as a Individual Language models then we have built final Label model on top of that using the label model we labelled 400k commit messages. we have balanced them properly. then we have Trained a Roberta Model based on that. we were able to achieve 76\% accuracy. Instead of Manual heuristic labeling methods to capture the positive commits, Our objective to build a model which understand the implicit features in the commit messages. we felt our labeling method should be robust. Large Language Models ability to understand the reasoning behind the commit messages could help to overcome. 

{ Idea- We can show case the Performance Metrics accuracy, precision, recall, F1 score in one diagram. one diagram for the Token/sec as it is performance efficiency of the Model on our gpu.}

In LLM approach, we have crafted a Perfect prompt to identify the performance commits. we have chosen Mistral 7B v2 Model.Initial Inference was performed by using Mistral 16 bit model which was proven to be slow for mining. so we have experimented with Quantized Mistral models such as AWQ \cite{}, gguf. we are using token per second to evaluate the efficiency of the Models on our gold validation dataset. so we have found that 16 bit mistral able to generate 1409 tokens/sec on 4090 GPU. Also, We have implemented the AWQ 4bit-quantization using Vllm library on our GPU server. mistral AWQ model single inference performance efficiency was 1573 tokens/sec.  we have used our prompt to label the commit messages. Using Mistral 16 bit Model with our custom prompt we were able to achieve 91\% Accuracy. Mistral taken quite long time for inference the commit messages even with Restricted output token limit to 5. compare to Roberta Mistral taken 85 times more time and 20 times computational memory. so,our new approach focused on Knowledge Distillation. Our Teacher model was mistral and student model was Roberta. we have taken 472k commit messages for the training. New Roberta Model Trained on Mistral supervision dataset. we were able to prove the Knowledge Distillation using Teacher model Mistral to Teach the student model so that the model performed 93.02\% on our gold validation dataset with the little trade off in the False Positive Rate. We have observed the FPR was slighly lower for the Roberta.  Roberta Model efficiency on the Gold label dataset was 17239 tokens/sec it was ~12 times faster than Mistral with GPU. Roberta consumes around 0.9 GB memory whereas Mistral consumes 23.20GiB Memory which is 26 times lesser than Mistral. Our objective to Mine performance data at scale so we are doing batch inference while mining the performance commits Roberta fits well for our task. 

\begin{table}[h!]
\centering
\small
\begin{tabular}{|l|c|c|c|c|c|}
\hline
Model                  & Accuracy & Precision & Recall  & F1 Score & FPR     \\ \hline
Roberta\_KD\_GPU  & 93.10\%  & 90.08\%   & 96.72\% & 0.93  & 10.44\% \\ \hline
Roberta\_HS\_GPU  & 76.27\%  & 77.25\%   & 73.77\% & 0.76  & 21.29\% \\ \hline
Roberta\_KD\_CPU  & 93.10\%  & 90.08\%   & 96.72\% & 0.93  & 10.44\% \\ \hline
Mistral\_GPU      & 91.17\%  & 91.70\%   & 90.39\% & 0.91  & 8.06\%  \\ \hline
Mistral\_AWQ\_GPU & 90.60\%  & 95.90\%   & 84.70\% & 0.90  & 3.57\%  \\ \hline
Mistral\_CPU      & 90.36\%  & 91.53\%   & 88.77\% & 0.90  & 8.07\%  \\ \hline
Mistral\_CPU\_GGUF  & 91.48\%  & 91.93\%   & 90.76\% & 0.91  & 7.82\%  \\ \hline
Regex\_Based     & 65.60\%  & 68.04\%   & 65.60\% & 0.64  & 16.00\%  \\ \hline
\end{tabular}
\caption{Performance Metrics of Various Models}
\label{table:performance_metrics}
\end{table}


Language Model Performance on CPU:

we wanted to understand the Performance of these Models on the CPU as we are doing Classification Task. Roberta consumes around 1.2 GB while doing Inference on the dataset with 2669 tokens/sec. similarly, Mistral Model on AMD Ryzen Threadripper PRO 5955WX 16-CoresCPU was 463 tokens/sec. which is very slow compared to Roberta on CPU. Our Method to choose a Large Language Model which fits our mining process at scale. so, we have explored different ways to mitigate this problem. Using V-LLM library we were able to use Mistral AWQ efficiently by implementing parallel inference on GPU. we will be creating a batch but when we do batch inference with AWQ mistral v2 was 100 times faster than single inference. Our objective to Mine performance data at scale so we are doing batch inference while mining the performance commits. 

\begin{table}[h!]
\centering
\small
\begin{tabular}{|l|c|c|}
\hline
Model                      & Tokens per Second & Memory Usage (GB) \\ \hline
Roberta\_KD\_GPU           & 17239.80      & 0.90          \\ \hline
Roberta\_HS\_GPU           & 18021.11      & 0.90          \\ \hline
Roberta\_KD\_CPU           & 2669.72      & 1.27        \\ \hline
Mistral\_GPU               & 1409.05       & 23.61         \\ \hline
Mistral\_AWQ\_GPU          & 1573.13       & 17.18      \\ \hline
Mistral\_CPU_Quantized     & 463.41        & 10.47         \\ \hline
Mistral\_CPU               & 62.29         & 34.27         \\ \hline
Regex\_Based               & 1694370.60         & 0.06              \\ \hline
\end{tabular}
\caption{Models Tokens per Second and Memory Usage on 4090x2 server with AMD Ryzen Threadripper PRO 5955WX 16-Cores}
\label{table:tokens_per_second_memory_usage}
\end{table}

 
\textbf{Comparative Analysis of Model Performance on 4090x2 Server vs. A10 Oracle Cluster} {Need to rewrite}

\subsubsection{Context}

To evaluate the performance of language models on implicit and explicit features, a dataset of 500 hand-labeled commit messages by two experts was used. This dataset includes 250 performance commits and 250 non-performance commits, serving as a gold standard for validation. The evaluation was conducted on two different hardware setups: a 2x4090 GPU server and an A10 Oracle cluster.

\subsubsection{Roberta Models}

On the 4090x2 server, the Roberta models (Roberta\_KD\_GPU and Roberta\_HS\_GPU) exhibit high tokens per second (TPS) rates, specifically 17,239.8 and 18,021.1 TPS respectively, while maintaining low memory usage of approximately 0.9 GB. This indicates that these models are highly efficient in processing speed and memory consumption on this hardware. Conversely, on the A10 Oracle cluster, the TPS for Roberta models decreases to 2,989.6, although memory usage remains the same. This suggests that while the A10 Oracle cluster is capable of handling the Roberta models, the performance efficiency is significantly reduced compared to the 4090x2 server.

\subsubsection{Mistral Models}

The Mistral models (Mistral\_GPU and Mistral\_AWQ\_GPU) show moderate TPS on the 4090x2 server, with 1,409.0 and 1,573.1 TPS respectively, but they require substantially more memory (23.6 GB and 17.2 GB). On the A10 Oracle cluster, the TPS for these models drops to 966.3, and the memory usage remains similar or slightly increases, highlighting the memory-intensive nature of the Mistral models. For the CPU versions, Mistral\_cpu achieves a TPS of 463.4 with 10.5 GB memory usage on the 4090x2 server, while the quantized version (Mistral\_cpu\_quantized) shows a drastically lower TPS of 62.3 but higher memory usage of 34.3 GB. These results indicate that the 4090x2 server is better suited for the memory-demanding Mistral models, whereas the A10 Oracle cluster’s limitations are more pronounced in handling these models efficiently.

\subsubsection{Regex\_Based Approach}

The Regex\_Based approach demonstrates exceptionally high TPS (1,694,370.6) with minimal memory usage (0.061 GB) on both setups. This emphasizes its efficiency for simple pattern matching tasks, despite lower accuracy and precision. This approach is highly effective for large-scale filtering tasks where speed is more critical than precision.

\subsubsection{Performance Metrics Summary}

Roberta models consistently show high accuracy, precision, and recall across both hardware setups. They are particularly efficient in terms of memory usage and TPS on the 4090x2 server, making them ideal for tasks requiring both speed and accuracy. Mistral models excel in precision and recall but at the cost of higher memory usage and lower TPS, making them more suitable for tasks where accuracy is paramount, and hardware constraints should be considered. The Regex\_Based method, while lower in accuracy, offers high efficiency in TPS and minimal memory usage, suitable for large-scale filtering tasks.

\begin{table}[h!]
\centering
\small
\begin{tabular}{|l|c|c|}
\hline
Model                      & Tokens per Second & Memory (GB) \\ \hline
Roberta\_KD\_GPU         & 13244.24     & 0.90    \\ \hline
Roberta\_HS\_GPU     & 13312 & 0.837    \\ \hline
Mistral\_GPU         & 890.63       & 15.86   \\ \hline
Mistral\_AWQ\_GPU    & 966.28        & 21.83   \\ \hline
Roberta\_KD\_CPU         & 2989.57       & 1.27    \\ \hline
Mistral\_cpu\    & 79.81         & 29.23  \\ \hline
Mistral\_cpu_Quantized    & 463.42        & 10.67   \\ \hline
Regex\_Based               & 1694370.60         & 0.06        \\ \hline
\end{tabular}
\caption{Model Names with Tokens per Second and Memory on A10 Oracle cluster}
\label{table:tokens_per_second_memory}
\end{table}

\begin{table}[h!]
\centering
\small
\begin{tabular}{|l|c|c|c|c|c|}
\hline
Model                  & Accuracy & Precision & Recall  & F1 Score & FPR     \\ \hline
Roberta\_KD\_GPU   & 93.10\%  & 90.08\%   & 96.72\% & 0.933  & 10.44\% \\ \hline
Roberta\_HS\_GPU  & 76.27\%  & 77.25\%   & 73.77\% & 0.76  & 21.29\% \\ \hline
Mistral\_GPU   & 90.56\%  & 95.81\%   & 84.70\% & 0.90  & 3.65\%  \\ \hline
Mistral\_AWQ\_GPU   & 90.56\%  & 95.81\%   & 84.70\% & 0.90  & 3.65\%  \\ \hline
Roberta\_CPU   & 93.10\%  & 90.08\%   & 96.72\% & 0.93  & 10.44\% \\ \hline
Mistral\_CPU\_GGUF   & 91.76\%  & 92.09\%   & 91.23\% & 0.92  & 7.71\%  \\ \hline
Mistral\_CPU       & 90.36\%  & 91.53\%   & 88.77\% & 0.90  & 8.07\%  \\ \hline
Regex\_Based     & 65.60\%  & 68.04\%   & 65.60\% & 0.64  & 16.00\%  \\ \hline
\end{tabular}
\caption{Performance Metrics of Various Models on A10 Oracle cluster}
\label{table:performance_metrics}
\end{table}


\subsection{Performance Bug Mining in the Wild}
Here we talk about our pipeline (Sketch a FIGURE of the pipeline)

\subsection{Dataset Cleaning}
\label{sebsection:dataset_collection}
Here we talk about data processing
\emph{Data Pre-processing}
\emph{Data Post-processing}
\emph{Deduplication} Data duplication can be a major problem in a dataset which may lead to unreliable model performance. To produce a high-quality dataset, we rigorously perform de-duplication during the data collection process. For each performance-related commit, we normalized the modified functions (before and after commits) by removing characters such as newline , spaces, tabs , and carriage return characters . We then compute the MD5 hash on the before and after commit versions of the function. We maintain a unique set of hashes during this process. Since our data collection process is distributed in nature, we further de-duplicate the dataset while merging the datasets from different curated on different nodes. This through de-duplication process will prevent the possibility of the training set leaking into the test dataset.

\subsection{Dataset description}
Here we talk about the collected data and meta-data



==> 7_related_works.tex <==
\section{Related Work}

\subsection{Existing approach to mining performance bugs} Here we talk about the papers that mines bug data based on keywords / talk about limited dataset, closed source . 

\subsection{Transformer-based approach for SE tasks} Here we talk about current usage of transformer/llms in SE Tasks
